Variance-weighted measurement planning and rank-aware adaptive precision for quantum subspace eigensolvers

Quantum subspace eigensolvers must control the joint sampling uncertainty of the projected Hamiltonian and overlap, not merely the number of measurement settings. We integrate variance-weighted commuting-Pauli grouping, independent paid-pilot Ritz replanning, and per-setting entangling-gate limits with a density-free, rank-aware adaptive precision controller. A preregistered study comprises \wpTotalAcq{} acquisitions and \wpTotalShotsB{} billion simulated physical shots on fixed eight- and ten-qubit molecular banks. Weighted sorted insertion meets the declared shot-cost and reliability criteria in \wpPoneaPassCount{}/\wpPoneaTotalCount{} matched-block comparisons, requiring \wpPoneaSpeedupMin{}--\wpPoneaSpeedupMax{} times fewer mean shots in the passing cells; the remaining cell ties on the discrete acquisition grid, so the global criterion fails. Paid-pilot replanning helps BeH\(_2\), but on LiH qubit-wise commuting (QWC) readout is cheaper than fully commuting readout, illustrating the limitations of state-independent variance proxies. Both weighted two-qubit-block arms meet the rank-stress criterion on stretched LiH, with no reduced-rank stops. An optional bootstrap-width guard instead incurs \wpWidthMeanRatioMin{}--\wpWidthMeanRatioMax{} times the mean shots, including \wpExhausted{} exhaustions. Tight noise gating meets all \wpPthreePassCount{}/\wpPthreeTotalCount{} relative two-qubit-noise criteria, but does not ensure absolute accuracy: the combined readout-noise regime produces \wpScFullBiasMin{}--\wpScFullBiasMax{}~mHa systematic bias in all arms, including QWC. These are simulations with fixed-bank energy targets, not hardware demonstrations or quantum advantage claims.

==> tables/p1_verdicts.tex <==
% Auto-generated by paper_weighted_precision/make_tables.py. Do not edit.
\multicolumn{8}{l}{\textit{Panel A: Predeclared P1a --- Weighted SI vs.\ unweighted LDF at matched $k$}} \\
\midrule
BeH$_2$ (8q) & $1$ & \texttt{si\_qwc} / \texttt{ldf\_qwc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & $0.0000$ (Yes) & $32/32$ ($1.000$) & \textbf{PASS} \\
BeH$_2$ (8q) & $2$ & \texttt{si\_k2} / \texttt{ldf\_k2} & $0.160$ $[0.160, 0.160]$ & $0.175$ $[0.160, 0.198]$ & $0.0000$ (Yes) & $32/32$ ($1.000$) & \textbf{PASS} \\
BeH$_2$ (8q) & $8$ & \texttt{si\_fc} / \texttt{ldf\_fc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & $0.0000$ (Yes) & $31/32$ ($0.806$) & \textbf{PASS} \\
LiH (8q) & $1$ & \texttt{si\_qwc} / \texttt{ldf\_qwc} & $0.064$ $[0.064, 0.064]$ & $0.074$ $[0.068, 0.083]$ & $0.0000$ (Yes) & $31/32$ ($0.806$) & \textbf{PASS} \\
LiH (8q) & $2$ & \texttt{si\_k2} / \texttt{ldf\_k2} & $0.160$ $[0.160, 0.160]$ & $0.180$ $[0.147, 0.217]$ & $0.0000$ (Yes) & $32/32$ ($1.000$) & \textbf{PASS} \\
LiH (8q) & $8$ & \texttt{si\_fc} / \texttt{ldf\_fc} & $1.000$ $[1.000, 1.000]$ & $1.000$ $[1.000, 1.000]$ & $1.0000$ (No) & $32/32$ ($1.000$) & \textbf{FAIL} (tie) \\
H$_4$ (8q) & $1$ & \texttt{si\_qwc} / \texttt{ldf\_qwc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & $0.0000$ (Yes) & $32/32$ ($1.000$) & \textbf{PASS} \\
H$_4$ (8q) & $2$ & \texttt{si\_k2} / \texttt{ldf\_k2} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & $0.0000$ (Yes) & $30/32$ ($0.480$) & \textbf{PASS} \\
H$_4$ (8q) & $8$ & \texttt{si\_fc} / \texttt{ldf\_fc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & $0.0000$ (Yes) & $32/32$ ($1.000$) & \textbf{PASS} \\
\midrule
\multicolumn{8}{l}{\textit{Panel B: Predeclared P1b (descriptive) --- Paid-pilot Ritz replanning vs.\ bank-weighted FC and QWC}} \\
\midrule
BeH$_2$ (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_fc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & RMSE $1.260$ & $32/32$ & $R/\hat{R} = 0.348$ \\
BeH$_2$ (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_qwc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & RMSE $1.260$ & $32/32$ & $R/\hat{R} = 0.348$ \\
BeH$_2$ (8q) & --- & \texttt{si\_fc} / \texttt{si\_qwc} & $1.000$ $[1.000, 1.000]$ & $1.000$ $[1.000, 1.000]$ & RMSE $1.319$ & $31/32$ & $R/\hat{R} = 0.209$ \\
LiH (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_fc} & $1.000$ $[1.000, 1.000]$ & $0.963$ $[0.906, 1.000]$ & RMSE $1.189$ & $32/32$ & $R/\hat{R} = 1.628$ \\
LiH (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_qwc} & $2.500$ $[2.500, 2.500]$ & $2.406$ $[2.266, 2.500]$ & RMSE $1.189$ & $32/32$ & $R/\hat{R} = 1.628$ \\
LiH (8q) & --- & \texttt{si\_fc} / \texttt{si\_qwc} & $2.500$ $[2.500, 2.500]$ & $2.500$ $[2.500, 2.500]$ & RMSE $1.113$ & $32/32$ & $R/\hat{R} = 1.397$ \\
H$_4$ (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_fc} & $1.000$ $[1.000, 1.000]$ & $1.000$ $[1.000, 1.000]$ & RMSE $1.133$ & $32/32$ & $R/\hat{R} = 0.547$ \\
H$_4$ (8q) & --- & \texttt{ritz\_si\_fc} / \texttt{si\_qwc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & RMSE $1.133$ & $32/32$ & $R/\hat{R} = 0.547$ \\
H$_4$ (8q) & --- & \texttt{si\_fc} / \texttt{si\_qwc} & $0.400$ $[0.400, 0.400]$ & $0.400$ $[0.400, 0.400]$ & RMSE $1.088$ & $32/32$ & $R/\hat{R} = 0.512$ \\


==> tables/p2_and_width.tex <==
% Auto-generated by paper_weighted_precision/make_tables.py. Do not edit.
\multicolumn{8}{l}{\textit{Panel A: Predeclared P2 --- Stretched 10-qubit LiH bank (10,341 words, rank 4, $\lambda_{\min}=0.10417$, $\tau_S=0.104$)}} \\
\midrule
\texttt{ldf\_qwc} & $15/16$ & $1$ ($0$) & $3.125$ / $4.883$ & baseline & $0.809$ & $16/16$ ($4.29$) & comparator \\
\texttt{si\_qwc} & $16/16$ & $0$ ($0$) & $3.125$ / $4.004$ & $0.820$ (ref.) & $0.620$ & $15/16$ ($3.17$) & comparator \\
\texttt{si\_k2} & $16/16$ & $0$ ($0$) & $3.125$ / $3.418$ & $0.700$ $[0.542, 0.927]$ & $0.705$ & $15/16$ ($3.21$) & \textbf{PASS} \\
\texttt{ritz\_si\_k2} & $16/16$ & $0$ ($0$) & $3.125$ / $4.004$ & $0.820$ $[0.593, 1.146]$ & $0.467$ & $16/16$ ($2.68$) & \textbf{PASS} \\
\midrule
\multicolumn{8}{l}{\textit{Panel B: Opt-in bootstrap half-width guard (\texttt{si\_fc\_width} vs.\ \texttt{si\_fc}) on 8-qubit banks}} \\
\midrule
BeH$_2$ (8q) & $28/32$ ($4$ exh.) & $0$ ($0$) & $3.906$ / $3.613$ & $5.781$ $[5.312, 6.133]$ & $0.506$ & $28/32$ ($28/28$ cond.) & $2.88\times$ boot \\
LiH (8q) & $31/32$ ($0$ exh.) & $1$ ($0$) & $3.906$ / $3.394$ & $5.430$ $[4.844, 5.898]$ & $0.535$ & $31/32$ ($31/32$) & $2.78\times$ boot \\
H$_4$ (8q) & $32/32$ ($0$ exh.) & $0$ ($0$) & $9.766$ / $9.033$ & $5.781$ $[5.312, 6.133]$ & $0.446$ & $31/32$ ($31/32$) & $2.88\times$ boot \\


==> tables/part_a_full.tex <==
% Auto-generated by paper_weighted_precision/make_tables.py. Do not edit.
BeH$_2$ (8q) & \texttt{ldf\_qwc} & $32/32$ & $25/7$ & $1.562$ / $1.562$ & $15.75$ & $1.484$ & $30/32$ ($7.11$) & $30/32$ ($6.96$) & $29/32$ ($5.21$) & $30/32$ ($5.10$) & $0.272$ \\
 & \texttt{si\_qwc} & $32/32$ & $30/2$ & $0.625$ / $0.625$ & $6.30$ & $0.899$ & $32/32$ ($4.72$) & $32/32$ ($5.43$) & $30/32$ ($3.46$) & $32/32$ ($3.98$) & $0.531$ \\
 & \texttt{ldf\_k2} & $32/32$ & $26/6$ & $1.562$ / $1.562$ & $16.25$ & $1.239$ & $31/32$ ($6.26$) & $32/32$ ($6.46$) & $31/32$ ($4.59$) & $31/32$ ($4.73$) & $0.217$ \\
 & \texttt{si\_k2} & $32/32$ & $24/8$ & $0.250$ / $0.273$ & $2.58$ & $1.362$ & $32/32$ ($7.54$) & $32/32$ ($7.91$) & $32/32$ ($5.53$) & $32/32$ ($5.79$) & $0.386$ \\
 & \texttt{ldf\_fc} & $32/32$ & $28/4$ & $1.562$ / $1.562$ & $17.26$ & $1.075$ & $32/32$ ($5.11$) & $32/32$ ($5.49$) & $30/32$ ($3.74$) & $30/32$ ($4.02$) & $0.171$ \\
 & \texttt{si\_fc} & $32/32$ & $26/6$ & $0.625$ / $0.625$ & $6.89$ & $1.319$ & $31/32$ ($6.92$) & $31/32$ ($7.15$) & $30/32$ ($5.06$) & $31/32$ ($5.24$) & $0.209$ \\
 & \texttt{ritz\_si\_fc} & $32/32$ & $25/7$ & $0.250$ / $0.250$ & $2.70$ & $1.260$ & $32/32$ ($5.87$) & $32/32$ ($6.48$) & $28/32$ ($4.30$) & $31/32$ ($4.74$) & $0.348$ \\
 & \texttt{si\_fc\_width} & $28/32$ ($4$) & $28/0$ & $3.906$ / $3.613$ & $43.05$ & $0.506$ & $28/32$ ($2.63$) & $28/32$ ($2.83$) & $26/32$ ($1.92$) & $27/32$ ($2.07$) & $0.208$ \\
\midrule
LiH (8q) & \texttt{ldf\_qwc} & $32/32$ & $26/6$ & $3.906$ / $3.394$ & $39.43$ & $1.352$ & $30/32$ ($5.53$) & $31/32$ ($5.77$) & $29/32$ ($4.05$) & $30/32$ ($4.22$) & $1.339$ \\
 & \texttt{si\_qwc} & $32/32$ & $25/7$ & $0.250$ / $0.250$ & $2.52$ & $1.511$ & $31/32$ ($7.79$) & $31/32$ ($8.13$) & $30/32$ ($5.70$) & $30/32$ ($5.95$) & $3.799$ \\
 & \texttt{ldf\_k2} & $32/32$ & $23/9$ & $1.562$ / $1.782$ & $16.18$ & $1.571$ & $31/32$ ($7.76$) & $32/32$ ($7.91$) & $28/32$ ($5.69$) & $29/32$ ($5.79$) & $1.367$ \\
 & \texttt{si\_k2} & $32/32$ & $25/7$ & $0.250$ / $0.320$ & $2.58$ & $1.450$ & $32/32$ ($7.38$) & $32/32$ ($8.17$) & $30/32$ ($5.41$) & $28/32$ ($5.98$) & $2.799$ \\
 & \texttt{ldf\_fc} & $32/32$ & $28/4$ & $0.625$ / $0.625$ & $6.87$ & $1.167$ & $31/32$ ($5.79$) & $32/32$ ($6.36$) & $30/32$ ($4.24$) & $29/32$ ($4.66$) & $1.501$ \\
 & \texttt{si\_fc} & $32/32$ & $26/6$ & $0.625$ / $0.625$ & $6.87$ & $1.113$ & $32/32$ ($5.89$) & $32/32$ ($6.42$) & $30/32$ ($4.32$) & $32/32$ ($4.70$) & $1.397$ \\
 & \texttt{ritz\_si\_fc} & $32/32$ & $27/5$ & $0.625$ / $0.602$ & $6.78$ & $1.189$ & $32/32$ ($5.90$) & $32/32$ ($5.76$) & $29/32$ ($4.32$) & $30/32$ ($4.22$) & $1.628$ \\
 & \texttt{si\_fc\_width} & $32/32$ & $31/1$ & $3.906$ / $3.394$ & $42.92$ & $0.535$ & $31/32$ ($2.49$) & $32/32$ ($2.53$) & $30/32$ ($1.83$) & $31/32$ ($1.85$) & $1.396$ \\
\midrule
H$_4$ (8q) & \texttt{ldf\_qwc} & $32/32$ & $25/7$ & $9.766$ / $9.766$ & $98.58$ & $1.341$ & $30/32$ ($5.97$) & $31/32$ ($6.21$) & $29/32$ ($4.37$) & $29/32$ ($4.55$) & $0.844$ \\
 & \texttt{si\_qwc} & $32/32$ & $21/11$ & $3.906$ / $3.906$ & $39.40$ & $1.482$ & $32/32$ ($7.06$) & $32/32$ ($7.90$) & $28/32$ ($5.17$) & $29/32$ ($5.79$) & $0.480$ \\
 & \texttt{ldf\_k2} & $32/32$ & $29/3$ & $9.766$ / $9.766$ & $101.11$ & $1.044$ & $31/32$ ($5.51$) & $32/32$ ($5.73$) & $30/32$ ($4.03$) & $30/32$ ($4.20$) & $0.669$ \\
 & \texttt{si\_k2} & $32/32$ & $27/5$ & $3.906$ / $3.906$ & $40.29$ & $1.443$ & $30/32$ ($6.88$) & $31/32$ ($7.62$) & $29/32$ ($5.04$) & $29/32$ ($5.58$) & $0.394$ \\
 & \texttt{ldf\_fc} & $32/32$ & $30/2$ & $3.906$ / $3.906$ & $44.18$ & $0.992$ & $32/32$ ($5.50$) & $32/32$ ($5.83$) & $31/32$ ($4.03$) & $31/32$ ($4.27$) & $0.468$ \\
 & \texttt{si\_fc} & $32/32$ & $27/5$ & $1.562$ / $1.562$ & $17.27$ & $1.088$ & $32/32$ ($6.42$) & $32/32$ ($6.62$) & $32/32$ ($4.70$) & $32/32$ ($4.85$) & $0.512$ \\
 & \texttt{ritz\_si\_fc} & $32/32$ & $26/6$ & $1.562$ / $1.562$ & $17.20$ & $1.133$ & $32/32$ ($6.13$) & $32/32$ ($6.18$) & $31/32$ ($4.49$) & $31/32$ ($4.53$) & $0.547$ \\
 & \texttt{si\_fc\_width} & $32/32$ & $32/0$ & $9.766$ / $9.033$ & $107.82$ & $0.446$ & $31/32$ ($2.62$) & $32/32$ ($2.61$) & $30/32$ ($1.92$) & $30/32$ ($1.92$) & $0.511$ \\
\midrule
LiH (10q, str.) & \texttt{ldf\_qwc} & $16/16$ & $15/1$ & $3.125$ / $4.883$ & $37.80$ & $0.809$ & $16/16$ ($4.29$) & $16/16$ ($5.43$) & $16/16$ ($3.08$) & $16/16$ ($3.90$) & $0.792$ \\
 & \texttt{si\_qwc} & $16/16$ & $16/0$ & $3.125$ / $4.004$ & $37.78$ & $0.620$ & $15/16$ ($3.17$) & $16/16$ ($3.70$) & $14/16$ ($2.28$) & $16/16$ ($2.66$) & $0.391$ \\
 & \texttt{si\_k2} & $16/16$ & $16/0$ & $3.125$ / $3.418$ & $38.72$ & $0.705$ & $15/16$ ($3.21$) & $16/16$ ($3.93$) & $14/16$ ($2.31$) & $16/16$ ($2.83$) & $0.325$ \\
 & \texttt{ritz\_si\_k2} & $16/16$ & $16/0$ & $3.125$ / $4.004$ & $38.63$ & $0.467$ & $16/16$ ($2.68$) & $16/16$ ($3.11$) & $15/16$ ($1.93$) & $15/16$ ($2.23$) & $0.330$ \\


==> tables/part_b_noisy.tex <==
% Auto-generated by paper_weighted_precision/make_tables.py. Do not edit.
BeH$_2$ (8q) & \texttt{depol2q\_p002} & \texttt{si\_qwc} & $312$ ($0$) & $16/0$ & $0.625$ & $0.000$ & $-0.344 \pm 0.804$ & $0.874$ & $15.5\%$ & $16/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $14$ ($7$) & $3/13$ & $0.625$ & $+2.841$ & $+2.828 \pm 1.307$ & $3.116$ & $82.4\%$ & $11/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $307$ ($1$) & $14/2$ & $0.625$ & $-0.520$ & $-0.608 \pm 0.856$ & $1.050$ & $33.5\%$ & $16/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $150$ ($3$) & $4/12$ & $0.625$ & $+2.498$ & $+2.673 \pm 1.384$ & $3.010$ & $78.9\%$ & $12/16$ &  \\
\midrule
BeH$_2$ (8q) & \texttt{depol2q\_p010} & \texttt{si\_qwc} & $312$ ($0$) & $10/6$ & $0.625$ & $0.000$ & $-0.412 \pm 1.484$ & $1.540$ & $7.2\%$ & $13/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $14$ ($7$) & $0/16$ & $0.625$ & $+13.820$ & $+13.282 \pm 0.966$ & $13.317$ & $99.5\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $307$ ($1$) & $2/14$ & $0.625$ & $-2.578$ & $-2.946 \pm 0.979$ & $3.104$ & $90.1\%$ & $7/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $150$ ($3$) & $0/16$ & $0.625$ & $+12.147$ & $+12.302 \pm 1.223$ & $12.362$ & $99.0\%$ & $0/16$ &  \\
\midrule
BeH$_2$ (8q) & \texttt{sc\_card\_full} & \texttt{si\_qwc} & $312$ ($0$) & $0/16$ & $0.625$ & $+61.783$ & $+61.843 \pm 1.215$ & $61.855$ & $100.0\%$ & $0/16$ & diag. \\
 &  & \texttt{si\_fc\_unc} & $14$ ($7$) & $0/16$ & $0.625$ & $+67.753$ & $+67.621 \pm 1.700$ & $67.643$ & $99.9\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $307$ ($1$) & $0/16$ & $0.625$ & $+62.414$ & $+62.592 \pm 0.949$ & $62.599$ & $100.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_mod} & $150$ ($3$) & $0/16$ & $0.625$ & $+67.857$ & $+68.097 \pm 1.307$ & $68.110$ & $100.0\%$ & $0/16$ &  \\
\midrule
LiH (8q) & \texttt{depol2q\_p002} & \texttt{si\_qwc} & $768$ ($0$) & $11/5$ & $0.273$ & $0.000$ & $+0.322 \pm 1.510$ & $1.544$ & $4.4\%$ & $14/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $59$ ($12$) & $3/13$ & $0.625$ & $+3.250$ & $+2.792 \pm 1.208$ & $3.042$ & $84.2\%$ & $11/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $720$ ($1$) & $15/1$ & $0.602$ & $-0.598$ & $-0.464 \pm 0.950$ & $1.057$ & $19.2\%$ & $16/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $282$ ($3$) & $1/15$ & $0.625$ & $+3.274$ & $+3.021 \pm 0.866$ & $3.143$ & $92.4\%$ & $11/16$ &  \\
\midrule
LiH (8q) & \texttt{depol2q\_p010} & \texttt{si\_qwc} & $768$ ($0$) & $11/5$ & $0.273$ & $0.000$ & $+0.230 \pm 1.684$ & $1.699$ & $1.8\%$ & $16/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $59$ ($12$) & $0/16$ & $0.625$ & $+15.555$ & $+15.798 \pm 1.558$ & $15.874$ & $99.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $720$ ($1$) & $4/12$ & $0.602$ & $-2.967$ & $-2.566 \pm 1.274$ & $2.865$ & $80.2\%$ & $8/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $282$ ($3$) & $0/16$ & $0.625$ & $+15.663$ & $+15.215 \pm 1.007$ & $15.248$ & $99.6\%$ & $0/16$ &  \\
\midrule
LiH (8q) & \texttt{sc\_card\_full} & \texttt{si\_qwc} & $768$ ($0$) & $0/16$ & $0.625$ & $+124.854$ & $+124.412 \pm 1.136$ & $124.417$ & $100.0\%$ & $0/16$ & diag. \\
 &  & \texttt{si\_fc\_unc} & $59$ ($12$) & $0/16$ & $1.562$ & $+134.882$ & $+134.365 \pm 1.180$ & $134.371$ & $100.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $720$ ($1$) & $0/16$ & $0.625$ & $+125.539$ & $+125.830 \pm 1.725$ & $125.841$ & $100.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_mod} & $282$ ($3$) & $0/16$ & $1.562$ & $+134.856$ & $+135.357 \pm 1.578$ & $135.366$ & $100.0\%$ & $0/16$ &  \\
\midrule
H$_4$ (8q) & \texttt{depol2q\_p002} & \texttt{si\_qwc} & $794$ ($0$) & $8/8$ & $3.906$ & $0.000$ & $+0.207 \pm 1.541$ & $1.555$ & $1.8\%$ & $16/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $61$ ($16$) & $2/14$ & $1.562$ & $+3.187$ & $+3.093 \pm 1.123$ & $3.290$ & $88.4\%$ & $8/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $745$ ($1$) & $12/4$ & $3.906$ & $+0.237$ & $+0.702 \pm 1.167$ & $1.362$ & $26.6\%$ & $16/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $297$ ($3$) & $2/14$ & $1.562$ & $+2.827$ & $+2.928 \pm 1.164$ & $3.151$ & $86.4\%$ & $11/16$ &  \\
\midrule
H$_4$ (8q) & \texttt{depol2q\_p010} & \texttt{si\_qwc} & $794$ ($0$) & $9/7$ & $3.906$ & $0.000$ & $+0.324 \pm 1.775$ & $1.804$ & $3.2\%$ & $14/16$ &  \\
 &  & \texttt{si\_fc\_unc} & $61$ ($16$) & $0/16$ & $1.562$ & $+14.853$ & $+14.587 \pm 0.963$ & $14.619$ & $99.6\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $745$ ($1$) & $9/7$ & $3.906$ & $+1.172$ & $+1.548 \pm 1.348$ & $2.052$ & $56.9\%$ & $13/16$ & \textbf{PASS} \\
 &  & \texttt{si\_fc\_mod} & $297$ ($3$) & $0/16$ & $1.562$ & $+13.285$ & $+13.055 \pm 1.790$ & $13.177$ & $98.2\%$ & $0/16$ &  \\
\midrule
H$_4$ (8q) & \texttt{sc\_card\_full} & \texttt{si\_qwc} & $794$ ($0$) & $0/16$ & $3.906$ & $+109.736$ & $+110.032 \pm 1.321$ & $110.040$ & $100.0\%$ & $0/16$ & diag. \\
 &  & \texttt{si\_fc\_unc} & $61$ ($16$) & $0/16$ & $1.562$ & $+114.980$ & $+114.376 \pm 1.301$ & $114.384$ & $100.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_tight} & $745$ ($1$) & $0/16$ & $3.906$ & $+109.806$ & $+109.439 \pm 1.626$ & $109.451$ & $100.0\%$ & $0/16$ &  \\
 &  & \texttt{si\_fc\_mod} & $297$ ($3$) & $0/16$ & $3.906$ & $+113.799$ & $+114.035 \pm 0.794$ & $114.037$ & $100.0\%$ & $0/16$ &  \\


==> tables/protocol_banks.tex <==
% Auto-generated by paper_weighted_precision/make_tables.py. Do not edit.
BeH$_2$ (8q) & $1,223$ & $3$ ($0.2106$; $0.005$) & $-15.560867$ & \texttt{ldf\_qwc} & $281$ & $2.15$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{si\_qwc} & $312$ & $3.78$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{ldf\_k2} & $37$ & $6.45$ & $108$ ($4$) & $1$ \\
 &  &  &  & \texttt{si\_k2} & $44$ & $14.13$ & $127$ ($4$) & $1$ \\
 &  &  &  & \texttt{ldf\_fc} & $12$ & $9.88$ & $71$ ($7$) & $5$ \\
 &  &  &  & \texttt{si\_fc} & $14$ & $18.11$ & $65$ ($7$) & $5$ \\
\midrule
LiH (8q) & $3,167$ & $3$ ($0.2106$; $0.005$) & $-7.863048$ & \texttt{ldf\_qwc} & $669$ & $2.09$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{si\_qwc} & $768$ & $7.28$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{ldf\_k2} & $278$ & $3.41$ & $517$ ($4$) & $1$ \\
 &  &  &  & \texttt{si\_k2} & $298$ & $19.49$ & $569$ ($4$) & $1$ \\
 &  &  &  & \texttt{ldf\_fc} & $61$ & $16.54$ & $343$ ($11$) & $6$ \\
 &  &  &  & \texttt{si\_fc} & $59$ & $26.07$ & $342$ ($12$) & $6$ \\
\midrule
H$_4$ (8q) & $3,051$ & $3$ ($0.2106$; $0.005$) & $-2.147929$ & \texttt{ldf\_qwc} & $701$ & $2.84$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{si\_qwc} & $794$ & $6.67$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{ldf\_k2} & $356$ & $4.32$ & $576$ ($4$) & $1$ \\
 &  &  &  & \texttt{si\_k2} & $399$ & $11.54$ & $598$ ($4$) & $1$ \\
 &  &  &  & \texttt{ldf\_fc} & $69$ & $16.29$ & $651$ ($18$) & $7$ \\
 &  &  &  & \texttt{si\_fc} & $61$ & $28.86$ & $432$ ($16$) & $7$ \\
\midrule
LiH (10q, str.) & $10,341$ & $4$ ($0.1042$; $0.104$) & $-7.763633$ & \texttt{ldf\_qwc} & $1,679$ & $2.92$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{si\_qwc} & $1,938$ & $8.27$ & $0$ ($0$) & $0$ \\
 &  &  &  & \texttt{si\_k2} & $490$ & $22.76$ & $1,294$ ($5$) & $1$ \\

